Quasiparticle properties of nonequilibrium gluon plasma

We apply classical gluodynamics to early stages of ultrarelativistic heavy-ion collisions. We start by going through the space-time evolution of ultrarelativistic heavy-ion collisions in the color glass condensate framework and the basics of real-time gluodynamics on the lattice in the temporal gauge. We study the plasmon mass scale in three- and two-dimensional systems by comparing three different methods to measure the mass scale. The methods are a formula which can be derived from Hard Thermal Loop effective theory at leading order (HTL), the effective dispersion relation (DR) and measurement of the plasma oscillation frequency triggered by the introduction of a uniform electric field (UE) into the system. We observe that in both systems the plasmon mass scale decreases like a power law after an occupation number dependent initial transient time. In both cases the UE and HTL methods are in rough agreement, and in the three-dimensional case the two agree in the continuum limit. As a second way to study the quasiparticle properties, we derive, implement and test an algorithm which can be used to simulate linearized fluctuations on top of the classical background. The algorithm is derived by requiring conservation of Gauss' law and gauge invariance. We then apply the algorithm to spectral properties of overoccupied gluodynamics using linear response theory. We establish the existence of transverse and longitudinal quasiparticles by extracting their spectral functions. We also extract the dispersion relation, effective mass, plasmon mass and damping rate of the quasiparticles. Our results are consistent with the HTL effective theory, but we also observe effects beyond leading order HTL.

==> papers.tex <==
\titleformat{\chapter}{}{}{0em}{\bf\Huge}


\addcontentsline{toc}{chapter}{{Papers I-IV}}
\cleardoublepage


%\chapter[Papers I-IV]{Paper I}

\ylatila

\noindent {\Huge \bf Paper I}



\mbox{} \\

\noindent \textbf{Time evolution of linearized gauge field fluctuations on a real-time lattice } \\
T. Lappi and J. Peuron, \\
\href{http://dx.doi.org/10.1140/epjc/s10052-016-4523-9}{\textit{Eur. Phys. J.} \textbf{C76} (2016) no. 12, 688}, \href{https://arxiv.org/abs/1610.01355}{\texttt{arXiv:1610.01355 [hep-lat]}}


\cleardoublepage
\pagestyle{empty}

\includepdf[pages={-}]{papers/flucts.pdf}

\cleardoublepage




\ylatila

\noindent {\Huge \bf Paper II}

\mbox{} \\

\noindent \textbf{Plasmon mass scale in classical nonequilibrium gauge theory 
} \\
T. Lappi and J. Peuron, \\ \href{http://dx.doi.org/10.1103/PhysRevD.95.014025}{\textit{Phys. Rev} \textbf{D95} (2017)  014025}, \href{https://arxiv.org/abs/1610.03711}{
	 \texttt{arXiv:1610.03711 [hep-ph]}}
	 
	 \cleardoublepage
	 
	 \includepdf[pages={-}]{papers/plasmon3.pdf}
	 
	 \cleardoublepage

\ylatila
	 
\noindent {\Huge \bf Paper III}

\mbox{} \\
	 \textbf{Plasmon mass scale in two dimensional classical nonequilibrium gauge theory } \\
	 T. Lappi and J. Peuron, \\	
	\href{http://dx.doi.org/10.1103/PhysRevD.97.034017}{\textit{Phys. Rev.} \textbf{D97} (2018) no.3, 034017}, 
	\href{https://arxiv.org/abs/1712.02194}{\texttt{arXiv:1712.02194 [hep-lat]}}
	
	
\cleardoublepage

	\includepdf[pages={-}]{papers/plasmon2.pdf}
	\cleardoublepage

\ylatila

\noindent {\Huge \bf Paper IV} 

\mbox{} \\
\textbf{Spectral function for overoccupied gluodynamics from real-time lattice simulations} \\
K. Boguslavski, A. Kurkela, T. Lappi and J. Peuron, \\
\href{https://doi.org/10.1103/PhysRevD.98.014006}{\textit{Phys. Rev.}  \textbf{D98}, 014006}
 \href{https://arxiv.org/abs/1804.01966}{\texttt{arXiv:1804.01966 [hep-ph]}} \\

	 
	 \cleardoublepage
	 
	 \includepdf[pages={-}]{papers/linfluct.pdf}

